The HOMFLY polynomial for links in rational homology 3-spheres

We construct a polynomial invariant, for links in a Seifert fibered or atoroidal rational homology 3-sphere, which generalizes the 2-variable Jones polynomial (HOMFLY). As a consequence, we show that the dual of the HOMFLY skein module of a homotopy 3-sphere is isomorpic to that of the genuine 3-sphere .

==> jmacros.tex <==


\magnification=1200
%\input mssymb.plain
\catcode`\@=11

\font\tenmsx=msam10
\font\sevenmsx=msam7
\font\fivemsx=msam5
\font\tenmsy=msbm10
\font\sevenmsy=msbm7
\font\fivemsy=msbm5
%\font\fivemsbm=msbm5
%\font\sevenmsbm=msbm7
\newfam\msxfam
\newfam\msyfam
%\newfam\msbmfam
\textfont\msxfam=\tenmsx  \scriptfont\msxfam=\sevenmsx
  \scriptscriptfont\msxfam=\fivemsx
\textfont\msyfam=\tenmsy  \scriptfont\msyfam=\sevenmsy
\scriptscriptfont\msyfam=\fivemsy
%\textfont\msbmfam=\sevenmsbm \scriptfont\msbmfam=\fivemsbm

\def\Bbb{\ifmmode\let\next\Bbb@\else
 \def\next{\errmessage{Use \string\Bbb\space only in math mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msyfam#1}

\baselineskip=15pt
%\footline={\tenrm  \phantom{a} \folio}
%\nopagenumbers
%\baselineskip=13pt
\font\small=cmr9 at 9pt
\font\Small=cmr7 at 7pt
\font\Smaller=cmr6 at 6pt
%\font\skata=cmr15 at 15pt
\font\msmall=cmr8 at 8pt
\font\vsmall=cmsl9 at 9pt


\def\picture #1 by #2 (#3){\vbox to #2{
    \hrule width #1 height 0pt depth 0pt
    \vfill
    \special{picture #3} % this is the low-level interface
} }

\def\scaledpicture #1 by #2 (#3 scaled #4){{
  \dimen0=#1 \dimen1=#2
  \divide\dimen0 by 1000 \multiply\dimen0 by #4
  \divide\dimen1 by 1000 \multiply\dimen1 by #4
  \picture \dimen0 by \dimen1 (#3 scaled #4)}
  }


\def\Z{{\Bbb Z}}
\def\Q{{\Bbb Q}}
\def\C{{\Bbb C}}
\def\R{{\Bbb R}}
\def\N{{\Bbb N}}

\overfullrule=0.0pt
\hsize=6.2truein
\hoffset=.3truein
\def\K{{\cal K}^{n}}
\def\c{{\cal K}^{n}_{c}}
\def\a{{\cal K}^{1}_{c}}
\def\b{{\cal K}^{j}_{c}}
\def\z{{\cal K}^{m}}
\def\h{{\cal K}^{m}_{c}}
\def\v{{\cal F}^{m}}
\def\n{{\cal F}^{m}_c}
\def\bg{{\cal K}^{(j,\ 1)}}
\def\d{{\cal K}^{(j,\ 1)}_c}
\def\om{{\Omega}^{j}}
\def\omc{{\Omega}^{j}_c}
\def\omo{{\Omega}^{(j,\ 1)}}
\def\omco{{\Omega}^{(j,\ 1)}_c}
\def\p{\noindent}
\def\Op{\mathop{\bigoplus}\limits}
\def\su{\mathop{\sum}\limits}
\def\qed {\nobreak$\quad$\lower 1pt\vbox{
    \hrule
    \hbox to 6pt{\vrule height 6pt\hfil\vrule height 6pt}
      \hrule}\ifmmode\relax\else\par\medbreak \fi}


